NPR: Nocturnal Place Recognition in Streets

Visual Place Recognition (VPR) is the task of retrieving database images similar to a query photo by comparing it to a large database of known images. In real-world applications, extreme illumination changes caused by query images taken at night pose a significant obstacle that VPR needs to overcome. However, a training set with day-night correspondence for city-scale, street-level VPR does not exist. To address this challenge, we propose a novel pipeline that divides VPR and conquers Nocturnal Place Recognition (NPR). Specifically, we first established a street-level day-night dataset, NightStreet, and used it to train an unpaired image-to-image translation model. Then we used this model to process existing large-scale VPR datasets to generate the VPR-Night datasets and demonstrated how to combine them with two popular VPR pipelines. Finally, we proposed a divide-and-conquer VPR framework and provided explanations at the theoretical, experimental, and application levels. Under our framework, previous methods can significantly improve performance on two public datasets, including the top-ranked method.

==> tables/disadvantages.tex <==
\begin{table}[hb]
\centering
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
Method                                         & VPR & LF &   (0.25m, 2\degree)   /   (0.5m, 5$\degree$)   /   (5m, 10\degree)    \\
\midrule
Baseline                                       &    &    & 64.3 \qquad \;  / 75.5 \qquad \; / 88.8 \\
\midrule
\multirow{2}{*}{+LIME\cite{lime}}                         &  $\checkmark$  &  $\checkmark$  & 60.2 (\textcolor{blue}{-4.1}) / 73.5 (\textcolor{blue}{-2.0}) / 83.7 (\textcolor{blue}{-5.1}) \\
                                               &    &  $\checkmark$  & 63.3 (\textcolor{blue}{-1.0}) / 74.5 (\textcolor{blue}{-1.0}) / 87.8 (\textcolor{blue}{-1.0}) \\
                                               \midrule
\multirow{2}{*}{+DUAL\cite{dual}}                         &  $\checkmark$  &  $\checkmark$  & 62.2 (\textcolor{blue}{-2.1}) / 73.5 (\textcolor{blue}{-2.0}) / 80.6 (\textcolor{blue}{-8.2}) \\
                                               &    &  $\checkmark$  & 64.3 \qquad \; / 73.5 (\textcolor{blue}{-2.0}) / 86.7 (\textcolor{blue}{-2.1}) \\
                                               \midrule
\multirow{2}{*}{+SIEN\cite{sien}}                         & $\checkmark$   &  $\checkmark$  & 55.1 (\textcolor{blue}{-9.2}) / 69.4 (\textcolor{blue}{-6.1}) / 79.6 (\textcolor{blue}{-9.2}) \\
                                               &    &  $\checkmark$  & 60.2 (\textcolor{blue}{-4.1}) / 75.5  \qquad \; / 88.8  \qquad \;\\
                                               \midrule
\multirow{2}{*}{+Zero-DCE\cite{zero}}                     &  $\checkmark$  & $\checkmark$   & 66.3 (\textcolor{red}{+2.0}) / 75.5 \qquad \; / 87.8 (\textcolor{blue}{-1.0}) \\
                                               &    & $\checkmark$   & 67.3 (\textcolor{red}{+3.0}) / 77.6 (\textcolor{red}{+2.1}) / 87.8 (\textcolor{blue}{-1.0}) \\ 
\bottomrule\\
\end{tabular}
}
\caption{\textbf{Results on the Aachen Day/Night dataset after applying different IE algorithms}.}
\label{disadvantage}
\end{table}
